Identification of Attack-Specific Signatures in Adversarial Examples

The adversarial attack literature contains a myriad of algorithms for crafting perturbations which yield pathological behavior in neural networks. In many cases, multiple algorithms target the same tasks and even enforce the same constraints. In this work, we show that different attack algorithms produce adversarial examples which are distinct not only in their effectiveness but also in how they qualitatively affect their victims. We begin by demonstrating that one can determine the attack algorithm that crafted an adversarial example. Then, we leverage recent advances in parameter-space saliency maps to show, both visually and quantitatively, that adversarial attack algorithms differ in which parts of the network and image they target. Our findings suggest that prospective adversarial attacks should be compared not only via their success rates at fooling models but also via deeper downstream effects they have on victims.

==> ablation.tex <==
\section{Ablation Studies}
\label{sec:ablation}

In this section, we evaluate our design choices for the proposed REDRL to better understand the contribution of Feature Reconstruction (FR) and Image Classification (IC) stages to the residual learning task. Therefore we compare the following three scenarios:

\begin{itemize}
    \item [A.] Here we ignore FR and IC stages and only optimize network $G$ for $\mathcal{L}_{R}(G)$ and $\mathcal{L}_{AC}(G)$.
    \item [B.] In this scenario, $\mathcal{L}_{F}$ is added so that network $G$ is optimized for $\mathcal{L}_{R}(G)$, $\mathcal{L}_{F}(G)$, and $\mathcal{L}_{AC}(G)$ objectives.
    \item [C.] We investigate the effect of image classification on the overall performance. Therefore, $G$ is trained for $\mathcal{L}_{R}(G)$, $\mathcal{L}_{IC}(G)$, and $\mathcal{L}_{AC}$ optimization functions.
\end{itemize}

Table \ref{tab:Ablation} presents how each step of the proposed REDRL can impact the downstream task of attack recognition. Note that in both CIFAR-10 and Tiny ImageNet datasets, REDRL consistently outperforms the rest of the scenarios in terms of overall attack detection accuracy. This shows that enforcing FR and IC constraints simultaneously helps to learn more representative residual. It is noteworthy to mention that we observe Image Classification module in REDRL significantly contributes to the high classification score on reconstructed images. 

\begin{table}[t!]
    \centering
    \caption{Investigating the effects of Feature Reconstruction ($\mathcal{L}_{F}$) and Image Classification ($\mathcal{L}_{IC}$) objectives on the adversarial attack recognition accuracy (\%).\\}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
         \cline{2-9}
         \multicolumn{1}{c|}{} & \multicolumn{8}{|c|}{Dataset} \\
         \cline{1-9}
         \multicolumn{1}{|c|}{\multirow{2}{*}{Class}} & \multicolumn{4}{|c||}{CIFAR-10} & \multicolumn{4}{|c|}{Tiny ImageNet}\\
         \cline{2-9}
         \multicolumn{1}{|c|}{} & \multicolumn{1}{|c|}{A} & \multicolumn{1}{|c|}{B} & \multicolumn{1}{|c|}{C} & \multicolumn{1}{|c||}{REDRL} & \multicolumn{1}{|c|}{A} & \multicolumn{1}{|c|}{B} & \multicolumn{1}{|c|}{C} & \multicolumn{1}{|c|}{REDRL}
         \\
         \cline{1-9}
         \multicolumn{1}{|c|}{Clean} & \multicolumn{1}{|c|}{$99.9$} & \multicolumn{1}{|c|}{$98.9$} & \multicolumn{1}{|c|}{$100$} & \multicolumn{1}{|c||}{$100$} & \multicolumn{1}{|c|}{$99.8$} & \multicolumn{1}{|c|}{$99.5$} & \multicolumn{1}{|c|}{$99.5$} & \multicolumn{1}{|c|}{$99.7$}
         \\
         \cline{1-9}
         \multicolumn{1}{|c|}{DeepFool} & \multicolumn{1}{|c|}{$99.3$} & \multicolumn{1}{|c|}{$98.8$} & \multicolumn{1}{|c|}{$99.8$} & \multicolumn{1}{|c||}{$97.4$} & \multicolumn{1}{|c|}{$87.1$} & \multicolumn{1}{|c|}{$93.8$} & \multicolumn{1}{|c|}{$71.9$} & \multicolumn{1}{|c|}{$75.3$}
         \\
         \cline{1-9}
         \multicolumn{1}{|c|}{PGD} & \multicolumn{1}{|c|}{$99.9$} & \multicolumn{1}{|c|}{$99.6$} & \multicolumn{1}{|c|}{$99.9$} & \multicolumn{1}{|c||}{$99.9$} & \multicolumn{1}{|c|}{$99.9$} & \multicolumn{1}{|c|}{$99.8$} & \multicolumn{1}{|c|}{$99.9$} & \multicolumn{1}{|c|}{$99.9$}
         \\
         \cline{1-9}
         \multicolumn{1}{|c|}{CW$L_2$} & \multicolumn{1}{|c|}{$84.2$} & \multicolumn{1}{|c|}{$88.7$} & \multicolumn{1}{|c|}{$93.3$} & \multicolumn{1}{|c||}{$96.6$} & \multicolumn{1}{|c|}{$58.7$} & \multicolumn{1}{|c|}{$60.2$} & \multicolumn{1}{|c|}{$61.5$} & \multicolumn{1}{|c|}{$66.3$}
         \\
         \cline{1-9}
         \multicolumn{1}{|c|}{CW$L_\infty$} & \multicolumn{1}{|c|}{$63.3$} & \multicolumn{1}{|c|}{$70.8$} & \multicolumn{1}{|c|}{$71.6$} & \multicolumn{1}{|c||}{$74.1$} & \multicolumn{1}{|c|}{$42.9$} & \multicolumn{1}{|c|}{$43.0$} & \multicolumn{1}{|c|}{$53.8$} & \multicolumn{1}{|c|}{$57.7$}
         \\
         \cline{1-9}
         \multicolumn{1}{|c|}{Patch} & \multicolumn{1}{|c|}{$99.7$} & \multicolumn{1}{|c|}{$99.8$} & \multicolumn{1}{|c|}{$99.9$} & \multicolumn{1}{|c||}{$99.9$} & \multicolumn{1}{|c|}{$98.6$} & \multicolumn{1}{|c|}{$98.9$} & \multicolumn{1}{|c|}{$99.2$} & \multicolumn{1}{|c|}{$99.6$}
         \\
          \hline
         \hline
         \multicolumn{1}{|c|}{Total} & \multicolumn{1}{|c|}{$90.59$} & \multicolumn{1}{|c|}{$92.58$} & \multicolumn{1}{|c|}{$93.51$} & \multicolumn{1}{|c||}{$\textbf{94.28}$} & \multicolumn{1}{|c|}{$81.9$} & \multicolumn{1}{|c|}{$82.7$} & \multicolumn{1}{|c|}{$83.72$} & \multicolumn{1}{|c|}{$\textbf{85.57}$}
         \\
         \cline{1-9}
    \end{tabular}
    }
    \label{tab:Ablation}
\end{table}


==> experiments.tex <==
\section{Experiments \& Results}
\label{sec:exp}
\Micah{MOVE THIS INTO THE SECTION ON REDRL}
\iffalse
In this section, we initially describe the datasets we use in our experiments. Next, we present the adversarial attacks employed to generate adversarial perturbations followed by the implementation details of the proposed reverse engineering of deceptions via residual learning. Finally, experimental results are reported.

\subsection{Datasets}
As previously mentioned, image classifier models have been frequently used in the context of adversarial attacks. We follow a similar practice. Additionally, prior works in the area of adversarial attacks have suggested investigating the effectiveness of designed methods through evaluation on datasets beside MNIST \cite{carlini2017adversarial, xu2019adversarial}. Therefore, in this study, we consider CIFAR-10 and Tiny ImageNet \cite{wu2017tiny} datasets to train and evaluate the proposed REDRL. Tiny ImageNet is a smaller subset of ImageNet benchmark \cite{deng2009imagenet} with $200$ object classes. The train and validation and test sets of Tiny ImageNet (CIFAR-10) contain $1e5$ ($4.5e5$), $1e4$ ($5e3$), and $1e4$ ($1e4$) images respectively. Compared to the CIFAR-10 dataset, the Tiny ImageNet has a higher diversity and larger dimensionality, \emph{i.e.} images are of the size $64\times64$. Therefore, it creates the opportunity to experiment on large-scale data while being more manageable than ImageNet in terms of computational resources.

\begin{table}
    \centering
    \caption{Image classification accuracy of different image classification models $\Phi$ over test set of \textbf{clean} samples for CIFAR-10 and Tiny ImageNet datasets.}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
         \cline{2-5}
         \multicolumn{1}{c|}{} & \multicolumn{4}{|c|}{Accuracy (\%)} \\
         \cline{1-5}
         \multicolumn{1}{|c|}{\multirow{2}{*}{Dataset}} & 
         \multicolumn{4}{|c|}{Model Architecture} \\
         \cline{2-5}
         \multicolumn{1}{|c}{} &
         \multicolumn{1}{|c|}{ResNet50} & \multicolumn{1}{|c|}{ResNext50} & \multicolumn{1}{|c|}{DenseNet121} & \multicolumn{1}{|c|}{VGG19} \\
         \hline
         \hline
         \multicolumn{1}{|c|}{CIFAR-10} & 94.02 & 94.76 & 94.48 & \multicolumn{1}{|c|}{95.73} \\
         \cline{1-5}
         \multicolumn{1}{|c|}{Tiny ImageNet}& 65.18 & 68.05 & 65.03 & \multicolumn{1}{|c|}{64.89} \\
         \hline
    \end{tabular}
    }
    \label{tab:image_classifier_details}
\end{table}

\subsection{Adversarial Attacks}
\label{subsec:adversarial_attacks}
To generate adversarial perturbations required for training and testing the proposed REDRL, we considered the following differentiable attacks:
\begin{itemize}
    \item \textbf{PGD}\cite{madry2017towards} produces $\delta$ in an iterative fashion in multiple steps. At each iteration, a gradual step is taken in the direction in which each image pixel should change to increase the loss function of a victim model. During this process, it is ensured that the generated adversarial sample $I_{adv}$ remains within the $\epsilon$-neighbor ball of the clean image $I_c$, \emph{i.e} $I_{adv}:{||I_{adv} - I_c||}_{\infty} \leq \epsilon$.
    \item \textbf{DeepFool}\cite{moosavi2016deepfool} attempts to iteratively find a route for $I_c$ to pass the decision boundary drawn by the image classification $\Phi$ model. Here, $\delta$ can be computed as the summation of perturbations (normal vector of the linearized decision boundary) found at each iteration.
    \item \textbf{CW} \cite{carlini2017towards} is a more subtle but computationally a more expensive approach to generate adversarial samples. Through a number of gradient descent iterations, CW seeks to find $I_{adv}$ that has the least distance measure to $I_c$ while fooling $\Phi$ to yield a higher logit value for a class different than the actual class of $I_c$. In this work, we consider $L_2$ and $L_\infty$ norms for the distance measure in the CW optimization. 
    
    \item \textbf{Adversarial Patch}\cite{karmon2018lavan}
    selects a random location within $I_c$ to be overlaid with a patch that its height and width are chosen from a range of $1/16$ to $1/4$ of the image height and width respectively. In addition, it is ensured that the crafted patch remains within the $\epsilon$-neighbor ball of the corresponding clean image content in the patch location. 
\end{itemize}
\fi




%\subsection{REDRL as a Defense Method}










